ZeroComp: Zero-shot Object Compositing from Image Intrinsics via Diffusion

We present ZeroComp, an effective zero-shot 3D object compositing approach that does not require paired composite-scene images during training. Our method leverages ControlNet to condition from intrinsic images and combines it with a Stable Diffusion model to utilize its scene priors, together operating as an effective rendering engine. During training, ZeroComp uses intrinsic images based on geometry, albedo, and masked shading, all without the need for paired images of scenes with and without composite objects. Once trained, it seamlessly integrates virtual 3D objects into scenes, adjusting shading to create realistic composites. We developed a high-quality evaluation dataset and demonstrate that ZeroComp outperforms methods using explicit lighting estimations and generative techniques in quantitative and human perception benchmarks. Additionally, ZeroComp extends to real and outdoor image compositing, even when trained solely on synthetic indoor data, showcasing its effectiveness in image compositing.

==> figures/fig_advantage_over_explicit_methods.tex <==
\begin{figure}[!th]
\centering
\scriptsize
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
    % \includegraphics[width=0.3\linewidth]{figures/advantage_over_explicit_methods/garon2019fast/9C4A0370-2d21311d85_02_crop_B075QDTYGK.png} & \includegraphics[width=0.3\linewidth]{figures/advantage_over_explicit_methods/karimidastjerdi2023everlight/9C4A0370-2d21311d85_02_crop_B075QDTYGK.png} & \includegraphics[width=0.3\linewidth]{figures/advantage_over_explicit_methods/iv_v2_06/9C4A0370-2d21311d85_02_crop_B075QDTYGK.png} \\
    \includegraphics[width=0.32\linewidth]{figures/advantage_over_explicit_methods/garon2019fast/AG8A6551-16ae8050c9_06_crop_B075X4QFK2.jpg} & \includegraphics[width=0.32\linewidth]{figures/advantage_over_explicit_methods/karimidastjerdi2023everlight/AG8A6551-16ae8050c9_06_crop_B075X4QFK2.jpg} & \includegraphics[width=0.32\linewidth]{figures/advantage_over_explicit_methods/op_v1_1.0_objdepth/AG8A6551-16ae8050c9_06_crop_B075X4QFK2.jpg} \\
    \includegraphics[width=0.32\linewidth]{figures/advantage_over_explicit_methods/garon2019fast/9C4A0307-ca23f47d11_00_crop_B075X5HB1D.jpg} &
    
    \includegraphics[width=0.32\linewidth]{figures/advantage_over_explicit_methods/karimidastjerdi2023everlight/9C4A0307-ca23f47d11_00_crop_B075X5HB1D.jpg}
    & \includegraphics[width=0.32\linewidth]{figures/advantage_over_explicit_methods/op_v1_1.0_objdepth/9C4A0307-ca23f47d11_00_crop_B075X5HB1D.jpg} \\
Garon'19~\cite{garon2019cvpr} & Everlight~\cite{dastjerdi2023everlight} & Ours
\end{tabular}
\caption{Advantage over explicit lighting estimation methods. Lighting estimation methods model the scene geometry with a simple plane \todo{is it always the case?}, which results in unrealistic shadows, whereas our method can realistically cast shadows using imperfect estimated scene depth. \todo{add arrows/crop to show shadows on walls}}
\label{fig:advantage_over_explicit_methods}
\end{figure}


==> figures/fig_qualitative_composition_methods.tex <==
\begin{figure*}[!t]
    \centering
    \tiny
    \setlength{\tabcolsep}{0.25pt}
    \renewcommand{\arraystretch}{0.25}
    \newlength{\customwidth}
    \setlength{\customwidth}{0.14\linewidth}
\begin{tabular}{ccccccc} 
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A9235-c076a13635_05_crop_B072PZJZY3_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg}\\  
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg}\\  
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A8626-28011c026e_00_crop_B07TYTPH77_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg}\\  
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A4861-19626f89e9_01_crop_B07QFP52CY_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg}\\  
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A9204-9e81794c27_01_crop_B002CM3J2A_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg}\\  
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A8542-042a892f91_09_crop_B07N2ZJYH6_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg}\\  
\includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A6765-55315335bf_07_crop_B0728NWFGY_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg}\\  
% \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1_bg.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/anydoor23/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/controlcom23/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/intrinsic_compositing23/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/arshadowgan20/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=\customwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg}\\  
Background & AnyDoor~\cite{chen2023anydoor} & ControlCom~\cite{zhang2023controlcom} & Careaga'23~\cite{careaga2023intrinsic} & ARSh.GAN~\cite{liu2020arshadowgan} & Ours & Simulated GT
 \end{tabular}
    \caption{Qualitative comparison with image-based compositing methods. Results are sorted from worst (top) to best (bottom) PSNR for ``Ours''. Please zoom in. Please refer to the \textbf{supplementary material} for additional images.}
    \label{fig:qualitative_comparison_composition_methods}
\end{figure*}


==> figures/fig_qualitative_lighting_methods.tex <==
\begin{figure*}[!ht]
    \centering
    \tiny
    \setlength{\tabcolsep}{0.25pt}
\renewcommand{\arraystretch}{0.25}
\begin{tabular}{cccccc} 
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A9235-c076a13635_05_crop_B072PZJZY3_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A9235-c076a13635_05_crop_B072PZJZY3.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A7811-8ad7ba9fd4_05_crop_B075YNL7R8.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A8626-28011c026e_00_crop_B07TYTPH77_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A8626-28011c026e_00_crop_B07TYTPH77.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A8500-0fc5c05bad_01_crop_B07DBF788Z.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A8378-92f902cb9a_06_crop_B07DBD9W9X.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A0132-07352d1dd0_06_crop_B07FJVXVRY.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A4861-19626f89e9_01_crop_B07QFP52CY_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A4861-19626f89e9_01_crop_B07QFP52CY.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A3196-8e1dfd8d95_04_crop_B07HPTBB7P_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A3196-8e1dfd8d95_04_crop_B07HPTBB7P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A3196-8e1dfd8d95_04_crop_B07HPTBB7P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A3196-8e1dfd8d95_04_crop_B07HPTBB7P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A3196-8e1dfd8d95_04_crop_B07HPTBB7P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A3196-8e1dfd8d95_04_crop_B07HPTBB7P.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A8088-1bb62eeb83_04_crop_B082VLJ7Y2.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A9204-9e81794c27_01_crop_B002CM3J2A_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A9204-9e81794c27_01_crop_B002CM3J2A.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A5577-970f71b3ac_07_crop_B07L6KPT9P.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/AG8A8542-042a892f91_09_crop_B07N2ZJYH6_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/AG8A8542-042a892f91_09_crop_B07N2ZJYH6.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A6765-55315335bf_07_crop_B0728NWFGY_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A6765-55315335bf_07_crop_B0728NWFGY.jpg}\\  
% \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/garon2019fast/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/karimidastjerdi2023everlight/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/weber2022editable/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/openrooms_wo_old_bboxdepth_depthscale1_v5/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_openrooms_wo_old_bboxdepth_depthscale1_v5_PSNR/GT_emission_envmap/9C4A9487-24b5ce36e4_01_crop_B07B4Y45N1.jpg}\\  
Background & Garon'19~\cite{garon2019cvpr} & Everlight~\cite{dastjerdi2023everlight} & Weber'22~\cite{weber2022editable} & Ours & Simulated GT
 \end{tabular}
    \caption{Qualitative comparison with lighting estimation methods. Results are sorted from worst (top) to best (bottom) PSNR for ``Ours''. Please zoom in. Please refer to the \textbf{supplementary material} for additional images.}
    \label{fig:qualitative_comparison_lighting_methods}
\end{figure*}


==> figures/fig_teaser.tex <==
% draw.io link: https://drive.google.com/file/d/1BxqgP3A1DJEu8pjsAGrQHztUtgyYh0RA/view?usp=share_link
\makeatletter
\g@addto@macro\@maketitle{
    \begin{figure*}[t]
    \centering
    \scriptsize
    \setlength{\linewidth}{\textwidth}
    \setlength{\hsize}{\textwidth}
    \vspace{-10mm}
    \footnotesize
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc}
        % \includegraphics[width=0.33\textwidth]{figures/teaser/teaser_render0001.png} &
        \includegraphics[width=0.32\textwidth]{figures/teaser/bg.jpg} & 
        \includegraphics[width=0.32\textwidth]{figures/teaser/obj-intrinsics.png} & 
        \includegraphics[width=0.32\textwidth]{figures/teaser/9C4A0370-2d21311d85_02_crop_B07QHYD995_pred_seed_1_comp.png}  \\
        % \includegraphics[width=0.32\textwidth]{figures/teaser/church_vase/dst_pixel_values.jpg} & 
        % \includegraphics[width=0.32\textwidth]{figures/teaser/church_vase/9C4A9274-cdf7c9a546_06_crop_B078JFFX4L_2.jpg} & 
        % \includegraphics[width=0.32\textwidth]{figures/teaser/church_vase/post_comp.jpg} \\
        % (a) target image &  (b) intrinsic maps & (c) predicted composite \\
    \end{tabular}
    \vspace{-5pt}
    \caption{From (a) a target background image and (b) available intrinsic maps (depth, normals, albedo) rendered from a 3D model, our method \method generates (c) a realistic composite, without access to the scene geometry or lighting, and without being trained specifically for object compositing. \method realistically shades the object and adds a compelling shadow.}    
    \label{fig:teaser}
    \vspace{-5pt}
	\end{figure*} 
}
\makeatother  

==> figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/results_figure2.tex <==
\begin{tabular}{cccccc} 
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/AG8A0630-e5622e17d2_01_crop_B07QJYKQ98_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/AG8A0630-e5622e17d2_01_crop_B07QJYKQ98.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/AG8A0630-e5622e17d2_01_crop_B07QJYKQ98.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/AG8A0630-e5622e17d2_01_crop_B07QJYKQ98.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/AG8A0630-e5622e17d2_01_crop_B07QJYKQ98.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/AG8A0630-e5622e17d2_01_crop_B07QJYKQ98.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/AG8A0630-e5622e17d2_02_crop_B075YMY1PD_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/AG8A0630-e5622e17d2_02_crop_B075YMY1PD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/AG8A0630-e5622e17d2_02_crop_B075YMY1PD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/AG8A0630-e5622e17d2_02_crop_B075YMY1PD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/AG8A0630-e5622e17d2_02_crop_B075YMY1PD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/AG8A0630-e5622e17d2_02_crop_B075YMY1PD.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A0370-2d21311d85_02_crop_B075QDTYGK_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A0370-2d21311d85_02_crop_B075QDTYGK.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A0370-2d21311d85_02_crop_B075QDTYGK.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A0370-2d21311d85_02_crop_B075QDTYGK.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A0370-2d21311d85_02_crop_B075QDTYGK.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A0370-2d21311d85_02_crop_B075QDTYGK.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A6864-533a74ab58_04_crop_B076VF4KRN_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A6864-533a74ab58_04_crop_B076VF4KRN.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A6864-533a74ab58_04_crop_B076VF4KRN.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A6864-533a74ab58_04_crop_B076VF4KRN.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A6864-533a74ab58_04_crop_B076VF4KRN.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A6864-533a74ab58_04_crop_B076VF4KRN.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/AG8A4408-86aa88feb2_03_crop_B07HGKV8JD_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/AG8A4408-86aa88feb2_03_crop_B07HGKV8JD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/AG8A4408-86aa88feb2_03_crop_B07HGKV8JD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/AG8A4408-86aa88feb2_03_crop_B07HGKV8JD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/AG8A4408-86aa88feb2_03_crop_B07HGKV8JD.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/AG8A4408-86aa88feb2_03_crop_B07HGKV8JD.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/AG8A4408-86aa88feb2_00_crop_B07Q2PGH2P_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/AG8A4408-86aa88feb2_00_crop_B07Q2PGH2P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/AG8A4408-86aa88feb2_00_crop_B07Q2PGH2P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/AG8A4408-86aa88feb2_00_crop_B07Q2PGH2P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/AG8A4408-86aa88feb2_00_crop_B07Q2PGH2P.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/AG8A4408-86aa88feb2_00_crop_B07Q2PGH2P.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A8088-1bb62eeb83_04_crop_B082VLTCM4_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A8088-1bb62eeb83_04_crop_B082VLTCM4.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A8088-1bb62eeb83_04_crop_B082VLTCM4.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A8088-1bb62eeb83_04_crop_B082VLTCM4.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A8088-1bb62eeb83_04_crop_B082VLTCM4.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A8088-1bb62eeb83_04_crop_B082VLTCM4.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A6639-4e986ca3a2_04_crop_B075X2WP64_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A6639-4e986ca3a2_04_crop_B075X2WP64.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A6639-4e986ca3a2_04_crop_B075X2WP64.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A6639-4e986ca3a2_04_crop_B075X2WP64.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A6639-4e986ca3a2_04_crop_B075X2WP64.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A6639-4e986ca3a2_04_crop_B075X2WP64.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/AG8A1520-f29e197a79_05_crop_B075X4PRNS_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/AG8A1520-f29e197a79_05_crop_B075X4PRNS.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/AG8A1520-f29e197a79_05_crop_B075X4PRNS.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/AG8A1520-f29e197a79_05_crop_B075X4PRNS.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/AG8A1520-f29e197a79_05_crop_B075X4PRNS.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/AG8A1520-f29e197a79_05_crop_B075X4PRNS.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A4475-8f1167988a_07_crop_B07B4ML473_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A4475-8f1167988a_07_crop_B07B4ML473.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A4475-8f1167988a_07_crop_B07B4ML473.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A4475-8f1167988a_07_crop_B07B4ML473.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A4475-8f1167988a_07_crop_B07B4ML473.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A4475-8f1167988a_07_crop_B07B4ML473.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/AG8A4702-1a77809d2c_01_crop_B07DBHFDSQ_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/AG8A4702-1a77809d2c_01_crop_B07DBHFDSQ.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/AG8A4702-1a77809d2c_01_crop_B07DBHFDSQ.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/AG8A4702-1a77809d2c_01_crop_B07DBHFDSQ.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/AG8A4702-1a77809d2c_01_crop_B07DBHFDSQ.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/AG8A4702-1a77809d2c_01_crop_B07DBHFDSQ.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A0608-306f35cf54_00_crop_B0871D4XPB_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A0608-306f35cf54_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A0608-306f35cf54_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A0608-306f35cf54_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A0608-306f35cf54_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A0608-306f35cf54_00_crop_B0871D4XPB.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A9487-24b5ce36e4_05_crop_B07RGKYS9K_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A9487-24b5ce36e4_05_crop_B07RGKYS9K.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A9487-24b5ce36e4_05_crop_B07RGKYS9K.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A9487-24b5ce36e4_05_crop_B07RGKYS9K.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A9487-24b5ce36e4_05_crop_B07RGKYS9K.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A9487-24b5ce36e4_05_crop_B07RGKYS9K.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A0608-306f35cf54_00_crop_B075X61W35_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A0608-306f35cf54_00_crop_B075X61W35.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A0608-306f35cf54_00_crop_B075X61W35.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A0608-306f35cf54_00_crop_B075X61W35.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A0608-306f35cf54_00_crop_B075X61W35.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A0608-306f35cf54_00_crop_B075X61W35.jpg}\\  
\includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/9C4A4878-4dac321d8b_06_crop_B075X5HBJ9_bg.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/garon2019fast/9C4A4878-4dac321d8b_06_crop_B075X5HBJ9.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/zhan2021emlight/9C4A4878-4dac321d8b_06_crop_B075X5HBJ9.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/arshadowgan20/9C4A4878-4dac321d8b_06_crop_B075X5HBJ9.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/controlcom23/9C4A4878-4dac321d8b_06_crop_B075X5HBJ9.jpg} & \includegraphics[width=0.16\textwidth]{figures/images_sorted_by_op_v1_1.0_objdepth_PSNR/op_v1_1.0_objdepth/9C4A4878-4dac321d8b_06_crop_B075X5HBJ9.jpg}\\  
\tiny{Background} & \tiny{Garon'19~\cite{garon2019cvpr}} & \tiny{EMLight~\cite{zhan2021emlight}} & \tiny{ARShadowGAN~\cite{liu2020arshadowgan}} & \tiny{ControlCom~\cite{zhang2023controlcom}} & \tiny{Ours}
 \end{tabular}


==> figures/old_fig_qual.tex <==
\begin{figure}[!ht]
    \centering
\begin{tabular}{ccccccccc} 
\rotatebox{90}{0-20} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/9C4A2563-d4a99744c5_00_crop_B07B8VJQG1.jpg}\\  
\rotatebox{90}{20-40} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/9C4A8378-92f902cb9a_06_crop_B07QGWMTDY.jpg}\\  
\rotatebox{90}{40-60} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/AG8A3196-8e1dfd8d95_08_crop_B07QFB5H6Y.jpg}\\  
\rotatebox{90}{40-60} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/9C4A8928-2fbd3aa74a_05_crop_B07HZ782D9.jpg}\\  
\rotatebox{90}{40-60} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/AG8A4408-86aa88feb2_05_crop_B07JM6HFW3.jpg}\\  
\rotatebox{90}{60-80} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/AG8A2294-51a6cdc9f8_06_crop_B072PZJZY3.jpg}\\  
\rotatebox{90}{60-80} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/AG8A9235-c076a13635_05_crop_B075YP32XY.jpg}\\  
\rotatebox{90}{60-80} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/9C4A7074-f46f94a5b1_04_crop_B07HPT2G8F.jpg}\\  
\rotatebox{90}{80-100} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/AG8A7219-5fb9e6b503_00_crop_B0871D4XPB.jpg}\\  
\rotatebox{90}{80-100} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_w_bg_bboxdepth/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_w_bg_bboxdepth/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/openrooms_wo_bg_bboxdepth/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/hypersim_wo_bg_bboxdepth/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/GT_emission_envmap/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/garon2019fast/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/gardner2019deep-1light/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg} & \includegraphics[width=0.12\textwidth]{figures/images_sorted_by_openrooms_wo_bg_bboxdepth_LPIPS/karimidastjerdi2023everlight/9C4A3419-2e5c9b4d85_00_crop_B07MF1S4YM.jpg}\\  
\rotatebox{90}{percentile of LPIPS on Ours} & \rotatebox{90}{Ours (Hypersim w/ BG)} & \rotatebox{90}{Ours (Openrooms w/ BG)} & \rotatebox{90}{Ours (Openrooms w/o BG)} & \rotatebox{90}{Ours (Hypersim w/o BG)} & \rotatebox{90}{Ground Truth} & \rotatebox{90}{Garon et al. 2019} & \rotatebox{90}{Gardner et al. 2019 (1 light)} & \rotatebox{90}{Everlight}
 \end{tabular}
    \caption{Qualitative comparison with other methods. Results are sorted by their quality based on LPIPS on the whole image on Ours (Openrooms w/o BG), i.e. the top images are more similar to the ground truth.}
    \label{fig:qualitative_comparison}
\end{figure}


==> sections/scratch.tex <==
\section{Experiments}
\label{sec:experiments}
In this section, we present a thorough evaluation of \method's capabilities as a neural renderer for zero-shot compositing. Our experiments are designed to highlight the robustness of ControlNet when trained solely for image rendering and its effectiveness in achieving zero-shot compositing. We demonstrate that our method performs on par with lighting estimation methods, yet without explicitly modeling lighting. Quantitatively and qualitatively, it outperforms other diffusion and intrinsic image-based baselines. Significantly, human evaluators prefer the results of our method, emphasizing its practical effectiveness over competitors. Further, we show our method's adaptability to real-world images and its potential to extend to tasks like image relighting.

\textbf{Reliable Neural Rendering with ControlNet}: Evidence that transforming ControlNet into a reliable neural renderer enhances zero-shot compositing capabilities.

\textbf{Training Focused on Rendering}: How training to render images is integral to achieving zero-shot compositing success.

\textbf{Performance Comparison}: Our method's competitive edge over lighting estimation-based approaches without explicitly predicting lighting conditions.

\textbf{Superiority Over Baselines}: A demonstration of our method's outperformance against other diffusion and intrinsic image-based baselines.

\textbf{Human Evaluation}: The insights gathered from human evaluations which confirm our method's superior performance compared to all baselines, a finding not fully captured by quantitative metrics alone.

\textbf{Generalization to Real Images}: Evidence supporting our method's ability to extend its applicability to real-world images beyond controlled dataset environments.

\textbf{Extension to Image Relighting}: Our exploration into how the Intrinsic ControlNet can be effectively utilized for image relighting tasks.

Each key takeaway will be discussed in detail, providing a comprehensive understanding of Intrinsic ControlNet's capabilities and advantages.

% Below, the actual subsections and further content will be developed with details of the experiments, results, and discussions.

